Quenching, bursting and galaxy shapes: colour transformation as a function of morphology

Different mechanisms for quenching star formation in galaxies are commonly invoked in the literature, but the relative impact of each one at different cosmic epochs is still unknown. In particular, the relation between these processes and morphological transformation remains poorly understood. In this work, we measure the effectiveness of changes in star formation rates by analysing a new parameter, the Star Formation Acceleration (SFA), as a function of galaxy morphology. This methodology is capable of identifying both bursting and quenching episodes that occurred in the preceding 300 Myrs. We use morphological classification catalogs based on Deep learning techniques. Our final sample has $\sim$14,200 spirals and $\sim$2,500 ellipticals. We find that elliptical galaxies in the transition region have median shorter quenching timescales ( $\tau$ < 1 Gyr) than spirals ($\tau \geq 1$ Gyr). This result conforms to the scenario in which major mergers and other violent processes play a fundamental role in galaxy evolution for most ellipticals, not only quenching star formation more rapidly but also playing a role in morphological transformation. We also find that $\sim$two thirds of galaxies bursting in the green valley in our sample are massive spirals ($M_\star \geq 10^{11.0}M_\odot$) with signs of disturbance. This is in accordance with the scenario where low mass galaxies are losing their gas in a interaction with a massive galaxy: while the former is quenching, the last is being refueled and going through a burst, showing signs of recent interaction.

==> Sections/Methodology.tex <==
\label{Chapter3}


\subsection{\textit{Star Formation Acceleration} -- SFA}
\label{subsec_sfa}

In order to quantify whether a galaxy is \textit{quenching} or \textit{bursting}, we use the parameter known as \textit{Star Formation Acceleration} (SFA), introduced by \citealp{martin2017quenching}. The SFA is a proxy for the instantaneous \textit{Star Formation Rate} (SFR) time derivative and is defined in equation \ref{eq_SFA}, where $(NUV-i)_0$ is corrected for extinction and $dt$ is the past 300 Myr:


\begin{equation}
    SFA \equiv \frac{d(NUV-i)_0}{dt},
    \label{eq_SFA}
\end{equation}
where SFA is measured in units of [mag Gyr$^{-1}$]. By definition, a positive SFA indicates that the galaxy is \textit{quenching} for the past 300 Myr, whereas a negative value indicates that the galaxy is \textit{bursting}. 

To obtain the SFA (and other physical parameters) \cite{martin2017quenching} used semi-analytical models (\citealp{de2006formation}) coupled up with the cosmological N-body \textit{Millenium} simulation (\citealp{springel2005simulations}) generating a catalogue of simulated galaxies that lies in redshift between $0~<~z~<~6$. 

Since the authors use a catalogue of mock galaxies, physical properties such as \textit{Star Formation Rate} (SFR), \textit{Star Formation History} (SFH), stellar mass, \textit{Star Formation Acceleration} (SFA) are known {\it a priori}. Observables (broadband colours and spectroscopic indices), on the other hand, are produced by using stellar population synthesis models. \citet{martin2017quenching} used models from (\citealp{bruzual2003stellar}) and a mixed extinction model -- that takes into account the star burst extinction law from \cite{calzetti2000dust} and the Milk Way extinction law (\citealp{cardelli1989relationship}) -- in order to produced synthetic spectra for each galaxy in the mock catalogue.

The simulated sample is then subdivided by $D_n(4000)$ and redshift, and in each bin a linear regression fit is performed between the physical properties and observables, generating a number of matrices of regression coefficients. This allows for later determination of physical properties from photometric and spectroscopic measurements of galaxies in observational surveys.

We used this methodology to infer SFA for the galaxy sample defined in Section \ref{Chapter2}. Although the determination of SFA is uncertain for single galaxies, given the standard deviation of $\sim 1$ Gyr$^{-1}$ in the linear regression in \citet{martin2017quenching}, the behaviour for a statistically significant sample is robust. For more details about the method, we refer the reader to \cite{martin2017quenching}.





